Weight Initialization of Deep Neural Networks(DNNs) using Data Statistics

Deep neural networks (DNNs) form the backbone of almost every state-of-the-art technique in the fields such as computer vision, speech processing, and text analysis. The recent advances in computational technology have made the use of DNNs more practical. Despite the overwhelming performances by DNN and the advances in computational technology, it is seen that very few researchers try to train their models from the scratch. Training of DNNs still remains a difficult and tedious job. The main challenges that researchers face during training of DNNs are the vanishing/exploding gradient problem and the highly non-convex nature of the objective function which has up to million variables. The approaches suggested in He and Xavier solve the vanishing gradient problem by providing a sophisticated initialization technique. These approaches have been quite effective and have achieved good results on standard datasets, but these same approaches do not work very well on more practical datasets. We think the reason for this is not making use of data statistics for initializing the network weights. Optimizing such a high dimensional loss function requires careful initialization of network weights. In this work, we propose a data dependent initialization and analyze its performance against the standard initialization techniques such as He and Xavier. We performed our experiments on some practical datasets and the results show our algorithm's superior classification accuracy.

==> ack.tex <==
%%%
\acknowledgments

\indent I would like to thank Prof. S.N. Merchant for granting me access to the SPANN lab and it's HPC server, the most of the work of this thesis would have been incomplete without it. I would also like to thank the keras\cite{keras} community. Almost each and every experiment has been programmed in python using keras deep learning library. Keras has been a big help for my work and none of this would have been possible without keras.






\signature{\today}
%\signature[Indian Institute of Technology Bombay]{\today}

%========================================================================

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../mainrep"
%%% End: 

==> dec.tex <==
%==================================dec.tex================================
%
\begin{Declaration}
\noindent
I declare that this written submission represents my ideas in my own words and where others' ideas or words have been included, I have adequately cited and referenced the original sources. I declare that I have properly and accurately acknowledged all sources used in the production of this report. I also declare that I have adhered to all principles of academic honesty and integrity and have not misrepresented or fabricated or falsified any idea/data/fact/source in my submission. I understand that any violation of the above will be a cause for disciplinary action by the institute and can also evoke penal action from the sources which have thus not been properly cited or from whom proper permission has not been taken when needed.

%
%
%
%
%
%
%

\DecSign[\today]



%
\end{Declaration}
%========================================================================

















